EvalResearchBench: Can AI Agents Build Their Own Feedback for Recursive Self-Improvement?

Recursive self-improvement (RSI) relies on evaluation feedback to assess progress and guide further research, yet repeatedly running complex benchmarks is costly and slows iteration. Human experts reduce this cost by selecting benchmark subsets or designing compact suites. We ask whether AI agents can automate this design process and introduce EvalResearchBench (ERB), a benchmark for autonomous evaluation research. Given target materials, development references, candidate APIs, and fixed time and API budgets, an agent called the researcher selects or synthesizes tasks, implements graders, and revises them in pilot tests before freezing an executable evaluator for coding, co-work, and reasoning. We study 9 researchers and 13 candidate models and compare each frozen evaluator with 14 target benchmarks on score concordance and pairwise agreement. The best evaluators order about 75\% of candidate pairs as the targets do, below the 91\% ceiling set by disagreements among the targets. No researcher leads on every metric, and the best evaluator on development targets is not the best on sealed targets hidden from the researcher. A human-designed sample of public tasks remains a strong baseline, and the evaluator with the lowest recorded execution cost attains the highest pairwise agreement. Agents repair tasks and graders through pilot feedback, yet their evaluators can still truncate answers, exhaust the evaluation budget, or let a few questions dominate a domain score.

==> figures/figure_ablation_random.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.92\linewidth]{figures/ablation-random-comparison.pdf}
\caption{\textbf{Available matched-panel diagnostic.} Random 30-question subset versus historical Astra on eleven targets, with the same 6--8 reference-bearing candidates per target. Lines connect two categorical conditions to aid comparison; they do not show a learning curve. The subset comes from the \$60-budget artifact rather than the historical Astra parent. This is a comparison between different designs, not a controlled estimate of an iteration or question-count effect.}
\label{fig:ablation-random}
\end{figure}


==> figures/figure_astra_outline.tex <==
\definecolor{outlineink}{HTML}{141413}
\definecolor{outlineaccent}{HTML}{D97757}
\definecolor{outlinepaper}{HTML}{F7F5F2}
\begin{figure}[!ht]
\centering
\fcolorbox{outlineaccent}{outlinepaper}{\begin{minipage}{0.94\textwidth}
\small
{\color{outlineink}\textbf{Astra's condensed evaluation-research loop}}\par\smallskip
\setlength{\tabcolsep}{5pt}
\begin{tabularx}{\linewidth}{@{}X X@{}}
{\color{outlineaccent}\textbf{01 Setup and coverage}} & {\color{outlineaccent}\textbf{02 Pilot and diagnose}}\\
Inspect targets, references, sources, and graders; organize $>$100 questions across three domains. & Test development candidates; identify truncation, brittle graders, and coverage gaps.\\[5pt]
{\color{outlineaccent}\textbf{03 Revise the instrument}} & {\color{outlineaccent}\textbf{04 Revise execution}}\\
Add miniature repositories; repair scientific fixtures and memo rubrics; accept valid alternatives. & Group compatible questions and revise allowances; retain selected short calls for discrimination.\\[5pt]
{\color{outlineaccent}\textbf{05 Audit and freeze}} & {\color{outlineaccent}\textbf{06 Independent assessment}}\\
Audit coverage, graders, and aggregation; distinguish explored changes from the submitted artifact. & Execute the frozen suite across candidates; compare domain scores with targets using Score and PA; record cost and completion.
\end{tabularx}
\end{minipage}}
\caption{\textbf{GPT-6-Astra research outline.} Decision types from construction and diagnosis to freezing; the last stage is the platform's independent assessment. This is not a count of iterations.}
\label{fig:astra-outline}
\end{figure}


==> figures/figure_case_study.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/sol-research-case.pdf}
  \caption{\textbf{Research trajectory and observed score-gap decomposition.} Top: selected stages of one Sol research episode. Bottom: an arithmetic decomposition of the Qwen--Astra co-work gap into task-group contributions on 59 completed tasks. Empty and truncated Astra responses dominate the gap; other tasks favor Astra. Values are rounded independently. Effective generation limits differed across routes.}
  \label{fig:sol-case}
\end{figure}


==> sections/k3_analysis.tex <==
K3's absolute-score agreement and pairwise order agreement vary by domain. A narrow score range and useful ordering can coexist; neither a high PA nor a low absolute error establishes statistical sensitivity to small differences among frontier models. The fixed-50 baseline illustrates why absolute error alone is insufficient.


==> sections/submission_statements.tex <==
\section*{AI Use Statement}
Generative AI tools assisted with research-methodology feedback, software implementation, analysis of execution traces, interpretation of results, and figure preparation. These uses are separate from the researcher agents and candidate models evaluated as experimental subjects. The reported numerical analyses use saved measurements and executable analysis scripts. The authors are responsible for the final text, claims, code, and artifacts, including AI-assisted contributions.

\section*{Ethics Statement}
This work studies automated evaluation design rather than experiments involving human participants. Generated tasks and graders can contain errors or encode biases; agreement with public reference scores does not establish broad validity or safety. Such evaluations should not be the sole basis for consequential deployment decisions. Credentials and private access information are excluded from the manuscript; redistribution of third-party tasks and traces remains subject to their source terms.

\section*{Reproducibility Statement}
Section~\ref{sec:method} specifies the research task, the submission contract, and independent assessment, and Section~\ref{sec:quality} defines the measured domain scores, Score, and PA. Section~\ref{sec:experimental-setup} and Table~\ref{tab:setup} list the researcher configurations and their harnesses, the candidate panel, the development and sealed splits, and all budgets. Appendix~\ref{app:matched-comparison} identifies the public leaderboard behind every reference score, the fixed reference scales, the candidate models, and per-target results; Appendix~\ref{app:cost-accounting} describes the cost accounting. Appendix~\ref{app:ablation-status} specifies the construction of Random120, including its sources, quotas, and sampling seed, together with the question-subset and candidate-resampling protocols, and Appendix~\ref{app:research-components} specifies the component-deletion and reweighting analyses. Appendix~\ref{app:prompts} describes the research instructions and the task interface given to researchers. All analyses beyond the frozen assessments reuse saved responses and make no new model calls.

